Pantograph: A Fluid and Typed Structure Editor

Structure editors operate directly on a program's syntactic tree structure. At first glance, this allows for the exciting possibility that such an editor could enforce correctness properties: programs could be well-formed and sometimes even well-typed by construction. Unfortunately, traditional approaches to structure editing that attempt to rigidly enforce these properties face a seemingly fundamental problem, known in the literature as viscosity. Making changes to existing programs often requires temporarily breaking program structure -- but disallowing such changes makes it difficult to edit programs! In this paper, we present a scheme for structure editing which always maintains a valid program structure without sacrificing the fluidity necessary to freely edit programs. Two key pieces help solve this puzzle: first, we develop a novel generalization of selection for tree-based structures that properly generalizes text-based selection and editing, allowing users to freely rearrange pieces of code by cutting and pasting one-hole contexts; second, we type these one-hole contexts with a category of type diffs and explore the metatheory of the system that arises for maintaining well-typedness systematically. We implement our approach as an editor called Pantograph, and we conduct a study in which we successfully taught students to program with Pantograph and compare their performance against a traditional text editor.

==> advantages.tex <==
\subsection{Advantages}
\label{sec:advantages}

\jacob{TODO: delete this section, move necessary parts to related work section.}

Beyond our immediate goal of designing a fluid structure editor, our contributions suggest new and interesting answers to some longstanding programming language questions.
In particular, a notable feature of Pantograph---that when one edits a part of the program, Pantograph modifies the rest of program in a particular way---allows for novel ways of facilitating type inference, type error blame, and refactoring actions.

For example, one common concern when designing statically typed languages is where to require type annotations.
Requiring annotations on all variables and parameters, like C, leads to users tediously providing redundant information. But inferring annotations through unification
can lead to difficulty pinpointing the location of the program responsible for the error
\cite{typeerrorlocation1} \cite{typeerrorlocation2} \cite{typeerrorlocation3},
and bidirectional type checking~\cite{bidirectional-type-checking} leads to difficult design decisions about where annotations are required.
\Naiive{} structure editors, such as Alfa~\cite{alfa} introduced a kind of dynamic inference---as one builds a term by filling holes, the type of the term is refined by unification without having to re-infer the type of the entire term.
However, this has the significant limitation that if one changes that term or its signature down the line, the type of the entire term needs to be re-checked from scratch and allow for type errors.
Pantograph offers a novel resolution that handles changes in types beyond refinement by unification---at every step of every edit in either a term or its signature, Pantograph accounts for the how the edit changes types and updates the corresponding signature or term respectively.

As another example, there is a large body of work on type error blame -- where to place errors in type checking/inference systems, such as \cite{blame}. 
Instead, Pantograph records \emph{how} a type changed from an edit with a diff, and uses this additional information to inform where to place error boundaries,
allowing for history-aware blaming of ill-typed code.
% This allows Pantograph to present errors messages more relevant to your edit history.

% \todo{diagram showing two edit sequences that end up at the same state (modulo type boundaries) where a normal text editor could not distinguish them, and so would put the error in the same place, but in Pantograph since it takes into account the history gives more useful errors by placing in different places}
% \leo{Again, probably no space}

%Overall, Pantograph presents a unified approach to supporting many features that have been considered useful and implemented ad-hoc in text-based editing systems.

% \paragraph{Contrast to checking (TODO)}


==> design.tex <==
\section{Design}
\label{sec:design}

The motivating constraints for Pantograph are:
\begin{itemize}
    \item well-formedness (i.e. be a structured editor) in every state
    \item well-typedness in every state
    \item fluid and complete edits
    \begin{itemize}
        \item fluid -- easy to edit a structure into a similar-looking structure
        \item complete -- easy to do every reasonable edit
    \end{itemize}
\end{itemize}

These constraints are broadly met by 1HC selection and type diffs.

\todo{Describe more formally the argument for this.}

\todo{write this section}

However, this still allows for many possible designs which answer these questions differently.

\subsection{Edit Actions}

\todo{write this section}
\todo{correspond edit action to those in text editor}

\begin{itemize}
    \item Hole fill - Given a cursor position $C[? : T_1]$ and a term $P : T_2$ where $T_1$ unifies with $T_2$ by $\sigma$, resulting program is $\sigma(C[P])$
    \item Hole dig - Given a cursor position $C[P]$, resulting program is $C[? : T]$
    \item Insert - Given a cursor position $C[P]$, and a one-hole context to be inserted $C' : \Delta \vdash d$, set up smallstep $C[\uparrow_{id \vdash d}\s{C'[\downarrow_{\Delta \vdash id}\s{P}]}]$
    \item Delete - Given a selection position $C_1[C_2[[P]]$, where $C_2 : \Delta \vdash d$, set up smallstep $C_1[\uparrow_{id \vdash d^{-1}}\s{C_2[\downarrow_{\Delta^{-1} \vdash id}\s{P}]}]$
\end{itemize}


\subsection{How are type-breaking changes handled?}

Pantograph maintains that every state is well-typed. But what if you want to have a temporarily ill-typed state? Some instances of this should be disallowed anyway e.g. if a hole has type $Int$ then you should not be able to fill it with $true$. Other instances appear to suggest it would be useful to allow for a temporarily badly-typed state, which should be made well-typed again by future edit e.g. if you dig the type signature of a definition, then the body should be marked as temporarily ill-typed (as opposed to replaced with a hole, which discards all the information in the body).

\begin{figure}
    \centering
    % TODO: \includegraphics{}
    \caption{What should happen when you dig the type signature of a definition?}
    \label{fig:dig-type-sig-for-temp-ill-typed}
\end{figure}

In Pantograph, this design choice amounts to how to handle the cases during rewriting when there is a boundary left in the state, but there is no base rewrite rule to continue propagating it.

\todo{I refer to the language-generic derived rewrite rules as the "base rewrite rules"}

The simplest option is to keep the base rewrite rules -- edits that result in an unresolved boundary get stuck, and so the edit is rejected.

We deemed that this approach is too restrictive in general, since in some cases for specific languages, such as in the example in \ref{fig:dig-type-sig-for-temp-ill-typed}, the edit should be allowed. We enumerated and handle these cases by extending the base rewrite rules with the custom language-specific rules in figure \ref{fig:rewrite-rules-for-introducing-boundaries}.

\begin{figure}
    \centering
    % TODO \includegraphics{}
    \caption{The base rewrite rules for TODO language are extended with these rules which can introduce boundaries into the state.}
    \label{fig:rewrite-rules-for-introducing-boundaries}
\end{figure}

This solution does not imply entirely abandoning Pantograph's goal of maintaining well-typedness in every state. These boundaries are an edit-time augmentation of a language's original syntax, along with new typing rules, and can only be introduced by the enumerated cases. Additionally, since these cases are handled via rewrite rules for editing, they take into account your edit history (it's not just re-checking your program after every edit). This defines a edit-aware blame system for where boundaries are placed.

\todo{implied edits related to boundaries (deleting a boundary)}

\subsubsection{Can local edits yield non-local changes?}

In Pantograph, edits are performed locally i.e. there is a cursor at a node of the AST where an edit is performed. However, its possible for edits to perform non-local modifications i.e. a part of the AST not immediately adjacent to the cursor is modified as a result of the edit. This non-local behavior is facilitated by the base rewrite rules, which propagates directional boundaries annotated by type diffs throughout the program. The goal of this propagation is to propagate the information about the new state of the program resulting from the local edit to other parts of the program that have types that are dependent on the types affected by the edit.

\todo{simple example to demonstrate type connected editing}

However, rather than propagate the boundaries immediately, an alternative design would be leave the boundaries in place. 

The actual menu of edits that the user has access to are defined language-specifically. So, an edit could create various up, down, or static boundaries for the same construct being inserted into the program, for example.

\todo{different ways or arranging boundaries around the result of an edit for inserting something e.g. lambda around body}

Main design options:
\begin{itemize}
    \item Immediately created boundaries are static and need to be resolved manually.
    \item Immediately created boundaries go up/down in various way from the local edit site.
    \item Propagating boundaries can have various rules for where they stop and become boundaries, perform non-local modifications.
\end{itemize}

We decided to include propagating boundaries with special rules about where  since there are many kinds of non-local edits that are obviously useful, take advantage of type diffs in interesting ways, and almost never do non-local modifications that are undesired.

\todo{interesting examples of non-local modifications being obviously useful}

There are some interesting design choices about which boundaries to send up/down.

\todo{other design options}

\subsection{User Interface}

\todo{}

\subsection{Trade-offs ("fire triangle")}

\todo{}

\subsection{Usefulness}

This section was part of the introduction but I moved it here:

We have developed an algebra of diffs between types, which type the one-hole contexts.

$$
C ::= C \to C \pipe + T \to [C] \pipe - T \to [C]
$$

For example, suppose that the user chooses to perform their edit by inserting the $\lambda.[]$ one hole context in the definition of the function. This is given the type diff $+ Int \to [Int]$. Our system propagates this diff through the program to perform the other two corresponding edits, as shown in the example. 
Therefore, the insertion of one-hole contexts not only preserve the grammar of the program, but also serve as semantically meaningful edits which can be handled by our typed-editing system.

Some edits in our system result in type errors being left in the program. For example, suppose that after adding the second argument to their function, the programmer decides that they didn’t want the first argument:

\includegraphics[scale=0.5]{sketches/intro5.PNG}

The programmer deletes the “h” argument. Our type-preserving edit system removes the argument from the type signature, but it can't unambiguously resolve the remaining reference to “h” in the function definition, nor the “[] 5” argument one-hole context at the call site. In both places, it simply leaves them in the program as type errors visible to the user. The user may choose to deal with those errors whenever they please, as the rest of the program is left intact and well-typed. 

A traditional typechecker would discover these type errors by checking the program after the edit was finished. However, it would not be able to recover all of this information; it wouldn't be able to tell if it were the first or second argument at the function call that had been deleted. Our editor system decides where to place the errors as part of the edit itself, which allows it to retain more information than a traditional typechecker separate from a code editor can know.


\begin{itemize}
    \item Argue for simplicity both with data and analogy to text editing
\end{itemize}

==> diffProofs.tex <==
\section{Diff Operation Theorems}
\label{app:groupoid}

Each of the following theorems is proven by straightforward induction over the four constructors of diffs that $d$ can have.

\begin{theorem}
    $$
        d^{-1} \circ d = d \circ d^{-1} = id
    $$
\end{theorem}

\begin{theorem}
    $$   
        id \circ d = d \circ id = d
    $$   
\end{theorem}

==> evaluation.tex <==
\section{Discussion}
\label{sec:discussion}

%In this section, we're will discuss advantages and disadvantages of our approach, showing how %Pantograph can handle the tasks of an existing case study \cite{tylr} focused on viscosity,
%before talking over the benefits and limitations of Pantograph at a high level.

%\input{advantages.tex}
\input{limitations.tex}

==> figures/generalize-indexed-map-typediffs.tex <==
\begin{figure}[H]
\label{fig:generalize-map-higher-order-typediffs}
\begin{framed}
\flushleft

% \begin{lstlisting}[frame=single]
% let map : (Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =
%     $\lambda$f : Bool $\to$ Bool . $\lambda$l : List Bool .
%     match l with
%         nil => nil
%         cons h t $\Rightarrow$ cons (f h) (map t) in
% map ($\hole$ : Bool $\to$ Bool) (cons 1 (cons 2 (cons 3)))
% \end{lstlisting}

Insert \code{\diff{Int \to}{}{}} at the type of \code{f}.

\begin{lstlisting}[frame=single]
let map : (Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =   
    (*@\hl{$\code{\uparrow (\diff{+ Int \to }{Bool \to Bool}{}) \to List~Bool \to List~Int}$ ~ [}@*)
    $\lambda$f : (*@\sethlcolor{green}\hl{$\code{Int \to }$}@*)Bool $\to$ Bool . (*@\hl{$\code{\downarrow \{ f : \diff{+ Int \to}{Bool \to Bool}{} \} ~ [}$}@*)$\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (f h) (map f t)(*@\hl{]}@*) (*@\hl{]}@*) in
map ($\hole$ : Bool $\to$ Bool) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}

Add a new argument hole to applications of \code{f} (figure \ref{fig:edit-generalize-map-typediffs} also showed handling adding a first order argument).

\begin{lstlisting}[frame=single]
let map : (Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =   
    (*@\hl{$\code{\uparrow (\diff{+ Int \to}{Bool \to Bool}{}) \to List~Bool \to List~Int}$ ~ [}@*)
    $\lambda$f : Int $\to$ Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (f(*@\hl{ ($\hole$ : $\code{Int}$)}@*) h) (map (f(*@\hl{ ($\hole$ : $\code{Int}$)}@*)) t)(*@\hl{]}@*) in
map ($\hole$ : Bool $\to$ Bool) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}

Change the signature of \code{map}. Traverse to the references to \code{map}.

\begin{lstlisting}[frame=single]
let map : ((*@\hl{$\code{Int \to }$ }@*)Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =   
    $\lambda$f : Int $\to$ Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (f ($\hole$ : $\code{Int}$) h) ((*@\hl{$\code{\uparrow (\diff{+ Int \to}{Bool \to Bool}{}) \to List~Bool \to List~Bool}$ ~ [}@*)map(*@\hl{]}@*) (f ($\hole$ : Int)) t) in
(*@\hl{$\code{\uparrow (\diff{+ Int \to}{Bool \to Bool}{}) \to List~Bool \to List~Bool}$ ~ [}@*)map(*@\hl{]}@*) ($\hole$ : $\code{Bool \to Bool}$) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}

Since the \code{\diff{+ Int \to }{Bool \to Bool}{}} is higher-order, traverse to the first argument applied to by \code{map}.

\begin{lstlisting}[frame=single]
let map : (Int $\to$ Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =   
    $\lambda$f : Int $\to$ Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (f ($\hole$ : $\code{Int}$) h) (map (*@\hl{$\code{\downarrow \diff{+ Int \to}{Bool \to Bool}{}}$[}@*)f ($\hole$ : Int)(*@\hl{]}@*) t) in
map (*@\hl{$\code{\downarrow \diff{+ Int \to}{Bool \to Bool}{}}$[}@*)($\hole$ : $\code{Bool \to Bool}$)(*@\hl{]}@*) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}

Insert a parameter to handle the type change.

\begin{lstlisting}[frame=single]
let map : (Int $\to$ Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =   
    $\lambda$f : Int $\to$ Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (f ($\hole$ : $\code{Int}$) h) (map ((*@\hl{$\lambda$ i : $\code{Int}$ . }@*)f ($\hole$ : Int)) t) in
map ((*@\hl{$\lambda$ i : $\code{Int}$ . }@*)($\hole$ : $\code{Bool \to Bool}$)) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}

\end{framed}

\caption{First edit of \code{map} to allow the mapped function to use the element index, with type diff annotations}
\end{figure}

==> figures/generalize-map-typediffs.tex <==
\begin{figure}[H]
\label{fig:generalize-map-typediffs}
\begin{framed}
\raggedright
\henry{I don't think we actually need to show the initial state, because it is implied by the first edit stuff, which highlights the things that have been augmented onto the initial state.}
% \begin{lstlisting}[frame=single]
% let map : List Bool $\to$ List Bool =
%     $\lambda$l : List Bool .
%     match l with
%         nil $\Rightarrow$ nil
%         cons h t $\Rightarrow$ cons (step h) (map t) in
% map (cons 1 (cons 2 (cons 3)))
% \end{lstlisting}
Add a parameter to \code{map}.
\begin{lstlisting}[frame=single]
let map : List Bool $\to$ List Bool =
    (*@\hl{$\uparrow$ $\code{\diff{+ (Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}}$\{}@*)(*@\sethlcolor{green}\hl{$\lambda$f : Bool $\to$ Bool . }@*)$\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (step h) (map t)(*@\hl{\}}@*) in
map (cons 1 (cons 2 (cons 3)))
\end{lstlisting}
Update the type signature of \code{map}.
\begin{lstlisting}[frame=single]
let map : (*@ \hl{$\code{(Bool \to Bool) \to }$} @*)List Bool $\to$ List Bool =
    (*@\hl{$\downarrow$ $\code{\{map : \diff{+ (Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}\}}$\{}@*)
    $\lambda$f : Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (step h) (map t) (*@\hl{\}}@*) in
(*@\hl{$\downarrow$ $\code{\{map : \diff{+ (Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}\}}$\{}@*) map (cons 1 (cons 2 (cons 3)))(*@\hl{\}}@*)
\end{lstlisting}
Traverse to the references to \code{map}.
\begin{lstlisting}[frame=single]
let map : (Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =
    $\lambda$f : Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (step h) ((*@\hl{$\uparrow$ $\code{\diff{+ (Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}}$\{}@*)map(*@\hl{\}}@*) t) in
(*@\hl{$\uparrow$ $\code{\diff{+ (Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}}$\{}@*)map(*@\hl{\}}@*) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}
Update the references to \code{map}.
\begin{lstlisting}[frame=single]
let map : (Bool $\to$ Bool) $\to$ List Bool $\to$ List Bool =
    $\lambda$f : Bool $\to$ Bool . $\lambda$l : List Bool .
    match l with
        nil => nil
        cons h t $\Rightarrow$ cons (step h) (map (*@\hl{ $\code{(\hole : Bool \to Bool)}$}@*) t) in
map(*@\hl{ $\code{(\hole : Bool \to Bool)}$}@*) (cons 1 (cons 2 (cons 3)))
\end{lstlisting}
\end{framed}
\caption{First edit of \code{map} to generalize it to use an input function, with type diff annotations}
\end{figure}


==> figures/insert_param_simple_diff_prop.tex <==
% \begin{figure}[H]
% \label{fig:insert_param_simple_diff_prop}


\begin{align*}
    &
    % \code{ \down{id, map : \plusdiffs{\cInt \to}{Bool \to Bool}{} \to id \; \vdash \; id}{map}~not~l }
    \code{\down{id,~ \code{map}: \plusdiffs{\cInt \to}{\cBool \to \cBool}{} \to id ~\vdash~ id}{\code{map}}~not~l}
    & (1)
    \\
    \textrm{\sc{Propagate-Var}} \downarrow 1\step &
    \code{\up{id \; \vdash \; \plusdiffs{\cInt \to}{Bool \to Bool}{} \to id}{map}~not~l }
    & (2)
    \\
    \textrm{\sc{Propagate-App}} \uparrow 1\step &
    \code{ \up{id \; \vdash \; id}{map~\down{id \vdash \plusdiffs{\cInt \to}{Bool \to Bool}{}}{not}}~l }
    & (3)
    \\
    \textrm{\sc{Identity}} \uparrow \step &
    \code{map~\down{id \vdash \plusdiffs{\cInt \to}{Bool \to Bool}{}}{not}~l }
    & (4)
    \\
    \textrm{\sc{Insert-Abs}} \downarrow\step &
    \code{ map~(\lambda \hole : Int~.~\downa{id \; \vdash \; \cBool \to \cBool}{not})~l }
    & (5)
    \\
    \textrm{\sc{Identity}} \downarrow \step &
    \code{ map~(\lambda \hole : Int~.~not)~l }
    & (6)
    \\
\end{align*}
    
% \caption{
% Updating the application of \code{map} by the context diff 
% $\code{id, map} : \plusdiff{\cInt \to}{\cBool \to \cBool}{} \to \cList\cBool \to \cList\cBool$.
% }

% \end{figure}

==> newmathsection.tex <==
\section{TITLE? New math section.}

In the previous section we showed how type diffs precisely encode how an edit changed the type of a term, and gave several examples of how Pantograph changes a program in response. In this section, we will describe how our system performs these automatic edits.

\subsection{Context diffs}

Reconsider Figure~\ref{fig:typed-editing-example-deleting-a-parameter}, where the user removes an argument from the \CC{map} function. In order to describe an alteration to the context like this, we introduce \emph{context diffs}, which we range over with $\Delta$.
Similarly to type diffs, we can represent the statement that a context diff $\Delta$ changes from context $\Gamma_1$ to context $\Gamma_2$ with the notation $ \Gamma_1 \xRightarrow{\Delta} \Gamma_2$.
Context diffs, shown below, consist of: an identity diff, which leaves the empty context $\varnothing$ unaltered; a variable diff $\Delta, x : \delta$, which allows the type of a variable $x$ in context to change by a type diff $\delta$; and context altering diffs that entirely add or remove a variable from the context.

\begin{align*}
    \Delta ~::=~        \varnothing \pipe
        \Delta, x : \delta \pipe
        \plusdiff{}{\Delta}{, x : T} \pipe
        \minusdiff{}{\Delta}{, x : T}
\end{align*}

When the user deletes the parameter from map in Figure~\ref{fig:typed-editing-example-deleting-a-parameter}, in addition to the type of \CC{map} changing, the context inside of the function changes as well; the type of \CC{map} loses an argument,  \CC{f} is removed from the context. This can be represented by a context diff:

\begin{align*}
\begin{array}{l}
\diffsto
    {\Gamma_1 }
    {\minusdiff{}{\varnothing, \code{map} : \minusdiff{(\cBool \to \cBool) \to}{\cList\cBool \to \cList\cBool}{}\;\;}{, \code{f} : (\cBool \to \cBool)}}
    {\Gamma_2} 
\\[1em]
\begin{array}{rl}
    \text{where} &
        \Gamma_2 = \varnothing, \code{map} : (\cBool \to \cBool) \to \cList\cBool \to \cList\cBool ,~ \code{f} : (\cBool \to \cBool) ,~ \varnothing
        \\ &
        \Gamma_1 = \varnothing, \code{map} : \cList\cBool \to \cList\cBool
\end{array}
\end{array}
\end{align*}

\subsection{Diff boundaries}

A type and context diff together give a full description for how the typing of a term needs to change.
Given a context diff $\Delta$ and a type diff $\delta$, we can put them together into a \emph{judgement diff} $\Delta \vdash \delta$.
Our typed editing system works by propagating these judgement diffs through the program.
%
% To achieve that, we introduce term-level syntax for the {\em diff boundaries} described in the  previous section:
To achieve that, we introduce term-level syntax for {\em diff boundaries}:
% Note from jacob: what do you mean described in the previous section?
\begin{align*}
    t ::= ~ ... \pipe 
        \down{\Delta \vdash \delta}{t} \pipe 
        \up{\Delta \vdash \delta}{t}
\end{align*}
%
The first form $\down{\Delta \vdash \delta}{t}$, called a \emph{down boundary}, represents the intention to alter $t$ by the context diff $\Delta$ and the type diff $\delta$. The second form on the other hand, called an \emph{up boundary}, can only be understood as a subexpression within a larger program. Given a one hole context $C$ into our program, $C \ohchole{\up{\Delta \vdash \delta}{t}}$ represents the intention to alter $C$ from the inside by $\Delta$ and $\delta$.

For example, if the user adds a parameter to a map function as in example 1 in Section~\ref{sec:typed-editing}, the system will set up the following configuration. The user's edit amounts to inserting a one-hole context $\lambda f : \cBool \to \cBool. \clasp{}$, and the system inserts a diff boundary above and below:

\begin{center}\begin{tabular}{c}\begin{lstlisting}
let map : List Bool $\to$ List Bool =
    $\{$ $\lambda f : \cBool \to \cBool .$
        $\{$ ... $\}_{\plusdiffs{}{id}{, f : \cBool \to \cBool} \vdash id}^\downarrow$
    $\}_{id \vdash \plusdiffs{(Bool \to Bool) \to}{List ~ Bool \to List ~ Bool}{}}^\uparrow$
in ...
\end{lstlisting}\end{tabular}\end{center}

The up boundary includes a type diff describing that the argument was inserted, while the down boundary includes a context diff representing that a variable was added to the context.

Pantograph performs typed edits by propagating these diff boundaries through the program.
In Pantograph, an edit begins with a one hole context that is added or removed from the program.

When the user makes an edit, there is some type and context at the cursor. In order to insert a one-hole context, the inner type and outer context must agree with those at the cursor. Then, the discrepancies in the typing are dealt with by inserting a type diff boundary going up above the insertion, and a context diff boundary going down below the insertion.

If the user inserts the one-hole context $C'$, typed $\Delta \vdash C' : \delta$, into the program $C[t]$, the system begins diff propagation with the setup $C[\up{id \vdash \delta}{C'[\down{\Delta ^{-1} \vdash id}{t}]}]$.
For example, if the user adds a parameter to a map function like example 1 in Section~\ref{sec:typed-editing}, the system will set up the following configuration:



\jacob{AAAAAAAAAAAAAAAAAAAAAAAAAAA}

As we described in Section~\ref{sec:general-diffs}, every one hole context can be understood as a list of single label steps c.
%
$$
C ::= \clasp{} \pipe c[C]
$$

For each step $c$, we write $\Delta \vdash c : \delta$ to represent that the context and type of $c$ change by diffs $\Delta$ and $\delta$ from the inside to the outside. A few language constructs have interesting diffs:

\begin{align*}
    \minusdiff{x : A ,~}{\Delta}{} &\vdash \fun{x}{A}{\clasp{}} : \plusdiff{A \to}{B}{}
    \\
    \Delta &\vdash \clasp{} \; t : \minusdiff{A \to}{B}{}
    % \\
    % \Delta & \vdash \errorboundary{T_1}{T_2}{ \clasp{} } : \replacediff{T_1}{T_2}
\end{align*}

For the rest of the steps in the language, we define the diffs across them to be either an identity diff if the type or context are the same between the outside and hole, or otherwise a replace diff.
%
We can describe the diffs across an entire one hole context by squashing together the diffs along the individual steps:

\begin{align*}
    \inferrule{
    }{
        id \vdash \clasp{} : id 
    }
    \hspace{3em}
    \inferrule{
        \Delta_2 \vdash c : \delta_2
        \\
        \Delta_1 \vdash C : \delta_1
    }{
        \Delta_1 \circ \Delta_2 \vdash c[C] : \delta_1 \circ \delta_2
    }
\end{align*}

\noindent
Diff propagation may result in
an up boundary at the top of the program. If this happens, Pantograph removes the boundary, and updates the type of the program accordingly. In this way, an edit can result in the type of the entire program changing.

==> oldtylrcase.tex <==
% \subsection{Tylr Case Studies}

% \label{sec:evaluation}

% In order to make a case that Pantograph allows common edits, we go through the four tasks used to evaluate Tylr \cite{tylr} in detail. While we did not run a user study, we show step by step how Pantograph can be used to perform each task.
% We believe that the examples show that our zipper editing system lends itself to making common edits in a straightforward way.
% % The fourth task involves type edits with interesting diffs, and we believe that this task also shows how Pantograph's automatic edits can be intuitive and useful.

% The first task involves wrapping a let around a function, and calling it. Figure \ref{fig:tylr-0} shows that this can be done by: (1) selecting the function, (2) inserting a let binding around it, and (3) filing in the remaining hole (the body of the let).

% % \begin{center}
% % \includegraphics[scale=0.3]{evaluationsketches/casestudy1.png}
% % \end{center}
% \begin{figure}
%     \begin{tikzpicture}
%         \node[draw] (step0) at (0,0) {\includepantographgraphics[0.22]{figures/tylr-0-step-0.png}};
%         \node[draw] (step1) at (4.5,0) {\includepantographgraphics[0.22]{figures/tylr-0-step-1.png}};
%         \node[draw] (step2) at (9.5,0) {\includepantographgraphics[0.22]{figures/tylr-0-step-2.png}};
%         % 
%         \draw[->,thick] (step0) to (step1);
%         \draw[->,thick] (step1) to (step2);
%     \end{tikzpicture}
%     \caption{Tylr case study 1: abstracting a constant to a function parameter.}
%     \label{fig:tylr-0}
% \end{figure}

% The second task is to relocate two let bindings inside a third. Figure \ref{fig:tylr-1} show how this can be done with a single zipper cut and paste.

% % \begin{center}
% % \includegraphics[scale=0.3]{evaluationsketches/casestudy2.png}
% % \end{center}

% \begin{figure}
%     \begin{tikzpicture}
%         \node[draw] (step0) at (0,0) {\includepantographgraphics{figures/tylr-1-step-0.png}};
%         \node[draw] (step1) at (6,0) {\includepantographgraphics{figures/tylr-1-step-1.png}};
%         % 
%         \draw[->,thick] (step0) to (step1);
%     \end{tikzpicture}
%     \caption{Tylr case study 2: rearranging definition scope.}
%     \label{fig:tylr-1}
% \end{figure}

% The third task begins with an expression with two complex subexpressions sharing similar structure. The goal is to factor out the shared structure into a function.
% Figure \ref{fig:tylr-2} show how this can be done as follows:
% First, the user creates a let binding and names it $f$. Next, using a zipper selection, the user cuts the shared part of the structure out of the expression and pulls it into the function. Another selection deletes the redundant structure on the other expression. Finally, the function is wrapped around both call sites.

% % \leo{Could we have some kind of delimiter in between steps? A horizontal line or something?}
% % \includegraphics[scale=0.3]{evaluationsketches/casestudy3.png}

% % \vspace{-1em}
% % \begin{center}
% \begin{figure}
%     \begin{tikzpicture}
%         \node[draw] (step0) at (0,0) {\includepantographgraphics[0.2]{figures/tylr-2-step-0.png}};
%         \node[draw] (step1) at (0,-1.2) {\includepantographgraphics[0.2]{figures/tylr-2-step-1.png}};
%         \node[draw] (step2) at (0,-2.6) {\includepantographgraphics[0.2]{figures/tylr-2-step-2.png}};
%         \node[draw] (step3) at (0,-4.0) {\includepantographgraphics[0.2]{figures/tylr-2-step-3.png}};
%         \node[draw] (step4) at (0,-5.4) {\includepantographgraphics[0.2]{figures/tylr-2-step-4.png}};
%         \node[draw] (step5) at (0,-6.8) {\includepantographgraphics[0.2]{figures/tylr-2-step-5.png}};
%         \node[draw] (step6) at (0,-8.2) {\includepantographgraphics[0.2]{figures/tylr-2-step-6.png}};
%         \node[draw] (step7) at (0,-9.6) {\includepantographgraphics[0.2]{figures/tylr-2-step-7.png}};
%         % 
%         \draw[->,thick] (step0) to node[right]{insert \CC{let}} (step1);
%         \draw[->,thick] (step1) to node[right]{select} (step2);
%         \draw[->,thick] (step2) to node[right]{cut and paste selection} (step3);
%         \draw[->,thick] (step3) to node[right]{select} (step4);
%         \draw[->,thick] (step4) to node[right]{delete selection} (step5);
%         \draw[->,thick] (step5) to node[right]{insert and use parameter} (step6);
%         \draw[->,thick] (step6) to node[right]{insert function calls} (step7);
%     \end{tikzpicture}
%     \caption{Tylr case study 3: abstracting a common operation to a function.}
%     \label{fig:tylr-2}
% \end{figure}
% % \end{center}
% % \vspace{-1em}

% The fourth task was to move two arguments from one function to another. This task differs from the others in that the variables referenced in the expression must change type by the end of the edits. Figure \ref{fig:tylr-3} shows how this can be done with a single zipper cut and paste if one were working in a setting where types weren't important.

% % \vspace{-1em}
% % \begin{center}
% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%         \node[draw] (step0) at (0,0) {\includepantographgraphics{figures/tylr-3-step-0.png}};
%         \node[draw] (step1) at (0,-1.2) {\includepantographgraphics{figures/tylr-3-step-1.png}};
%         % 
%         \draw[->,thick] (step0) to (step1);
%     \end{tikzpicture}
%     \caption{Tylr case study 4: rearranging arguments (untyped).}
%     \label{fig:tylr-3}
% \end{figure}
% % \end{center}
% % \vspace{-1em}

% On the other hand, Pantograph keeps track of types. Figure \ref{fig:tylr-4} shows how the user can perform the edit by first cutting and pasting the two arguments from the signature of $h$ to the signature of $f$. This creates two holes in the call to $f$, and the two arguments to $g$ are commented out since they no longer fit. Finally, the user cuts and pastes the terms into their new positions to finish the edit.

% % \begin{center}
% % \includegraphics[scale=0.35]{evaluationsketches/casestudy4types.png}
% % \end{center}

% \begin{figure}
%     \begin{tikzpicture}
%         \node[draw] (step0) at (0,0) {\includepantographgraphics{figures/tylr-4-step-0.png}};
%         \node[draw] (step1) at (0,-2.3) {\includepantographgraphics{figures/tylr-4-step-1.png}};
%         \node[draw] (step2) at (0,-4.6) {\includepantographgraphics{figures/tylr-4-step-2.png}};
%         % 
%         \draw[->,thick] (step0) to node[right]{cut and paste selection} (step1);
%         \draw[->,thick] (step1) to node[right]{cut and paste terms} (step2);
%     \end{tikzpicture}
%     \caption{Tylr case study 4: rearranging arguments (typed).}
%     \label{fig:tylr-4}
% \end{figure}

==> outline.tex <==
\section*{Outline}

\begin{itemize}
    \item introduction
    \begin{itemize}
        \item structure editing is editing the source as a tree
        \item the naive structure editor is augmenting the syntax with typed holes
        \begin{itemize}
            \item properties: well-formedness, well-typedness
            \item examples: Alfa, Scratch, Lambdu, ...
            \item good for building programs from scratch
        \end{itemize}
        \item problem: editing existing code is cumbersome -- viscosity problem in structure editing
        \item previous approaches: trade-off original structure editing goals for more fluidity by allowing user to temporarily violate well-formedness or well-typedness
        \item our approach: with some novel insights, we can adhere to the original goals of structure editing without compromising fluidity
        \begin{itemize}
            \item user can select and edit in terms of 1HCS
            \begin{itemize}
                \item is an extension of the naive structure editor in an analogous way to selection in text editing
                \item facilitates fluid editing
            \end{itemize}
            \item problem: by itself, 1HC edits doesn't do anything to maintain well-typedness
            \begin{itemize}
                \item we present a type system that correspond 1HC edits to type diffs that encodes how the program should change to account for the change in types caused by the 1HC edit
            \end{itemize}
        \end{itemize}
        \item contributions:
        \begin{itemize}
            \item zipper editing extends the naive structure editor with 1HC edits to improve fluidity while maintaining well-formedness
            \item typed editing accounts for type changes by 1HC edits to maintain well-typedness and fluidity
            \item  Pantograph implements typed editing for an SML-like language
        \end{itemize}
    \end{itemize}
    \item zipper editing
    \begin{itemize}
    \item define SML-like language syntax
        \item show how its cumbersome to manipulate existing code in the naive structure editor
        \item 1HC selections generalize selection to trees
        \begin{itemize}
            \item cursor in text editor :: cursor in naive structure editor
            \item selection in text editor :: 1HC selection in extended structure editor
        \end{itemize}
        \item walkthrough examples of editing with 1HCs
        \begin{itemize}
            \item example: reorder parameters by cutting/pasting lambdas
            \item example: generalize \code{map} to be over an arbitrary function
        \end{itemize}
    \end{itemize}
    \item typed editing
    \begin{itemize}
        \item semantic interpretation of 1HC edits
        \item problem: a 1HC edit can result in an ill-typed program
        \item solution: system of type diffs to formalize how types should change according to the 1HC edit
        \item high-level definition of type diffs
        \item simple example of associating 1HC with a type diff
        \item example editing with type diffs:
        \begin{itemize}
            \item add parameter to \code{map} (this corresponds to the first edit from the \code{map} example in the zipper editing section)
            \item add higher-order parameter to the first parameter of \code{map} (demonstrates novel generality of type diff system over traditional refactoring)
        \end{itemize}
    \end{itemize}
    \item editor design
    \begin{itemize}
        \item Advantages
        \begin{itemize}
            \item adhere to original goals of structure editing: well-formedness, well-typedness
            \item improve fluidity by letting the user make any (reasonable) change they want, and then modifying the surrounding program to account for that
            \item type boundaries
            \item non-local changes
        \end{itemize}
        \item custom rules
        \begin{itemize}
            \item TODO
        \end{itemize}
        \item Disadvantages/ Limitations [jacob]
        \begin{itemize}
            \item zipper editing doesn't handle associative structures well
            \item type diffs don't deal with curried applications with partial applications well (but it works fine with just zipper editing)
            \item trade-offs for type diff system
        \end{itemize}
        \item evaluation
        \begin{itemize}
            \item Go through tylr user study examples, show how they work in Pantograph.
            \begin{itemize}
                \item advantages of structure editors without downside of 
                \item edit history aware feedback
            \end{itemize}
        \end{itemize}
    \end{itemize}
\item related work [henry]
\begin{itemize}
    \item Hazel/Tylr: compromised structure editing in order to achieve fluidity
    \item include references to other related work
    \item recent Hazel papers
    \item show how previous approaches are basically all the same "simple" structure editors (include Isomorph)
\end{itemize}
\item future work
\begin{itemize}
    \item user study
    \item more advanced type systems
    \item stronger theoretical results about language-generic editing semantics
\end{itemize}

\end{itemize}


==> revisionchanges.tex <==
We have included two PDFs: one is the updated version of the paper, and another is the updated version of the paper annotated with what has changed since the original submission.
The blue-outlined parts are additions from the previous version, and the green-outlined parts are artifacts of the PDF diff tool we used that signify text that moved across pages (and so can be ignored).

Overall, we implemented all proposed changes. Other than minor fixes in wording, the only additional change was that we added "Intrinsically-typed" to the title to emphasize even further the distinction 
between Pantograph and other editors. We feel that it conveys the content of the paper 
better after considering the post-rebuttal additions, but don't feel too strongly 
if reviewers are opposed for some reason.

% ---------------------------------------------------------------
- Required Change #1: Clearer motivation for intrinsically typed editors in the introduction

We added a prominent paragraph at the end of the introduction to motivate intrinsically typed editing on lines 159 - 167.

% ---------------------------------------------------------------
- Required Change #2: Explicitly mention existence of type boundaries in introduction

We described the existence of explicit type error forms on lines 162 and 165.
We also mentioned them again to qualify "well-typedness" on line 172.

% ---------------------------------------------------------------
- Required Change #3: A qualitative analysis of the user study

User Study Qualitative Analysis:

Following your suggestion, we performed a reflexive thematic analysis following the six step process outlined in Braun and Clarke.
We wrote section 6.2 (lines 1055 - 1137) describing the results of this analysis.
Thanks again for the suggestion - it was really helpful!

% ---------------------------------------------------------------
- Required Change #4: Additional discussion of the eval limitations w.r.t. other editors

We clarified the text in the beginning of the user study section (955), and again explicitly mention the goals of the study and discuss the (lack of a) comparison with other structure editors in the
limitations section (6.3, 1142, 1169).

% ---------------------------------------------------------------
- Required Change #5: Also for discussion of eval limitations: Everything acknowledged in the response about the large potential for bias in the study outcome

We included all the rebuttal points and those raised by reviewers in the limitations section (6.3),
including comparison with other editors as above (1142, 1169); short time to practice with 
Pantograph (1144); users were aware we created Pantograph (1156); we conducted the tutorial
and different teachers could lead to non-reproducibility (1158); allowing for questions (1160).



In particular: 
Line 1141: Our results lend little insight to how our system compares to other structure editors.
Line 1144: A potential source of bias is that participants only got a relatively (to Pantograph) short time to practice using the language in the text editor.
Line 1156: Our results have a large potential for bias and non-reproducibility.
Lines 1158 - 1160 : Different teachers in the tutorial and allowing questions during tasks could lead to non-reproducibility
Line 1163: We only claim to demonstrate our approaches feasibility rather than its effectiveness compared to other state of the art structure editors or text editors.


==> smallsteprules.tex <==
\begin{figure}
\begingroup
\renewcommand{\arraystretch}{1.5} % Default value: 1
\newcolumntype{R}{>{$}r<{$}}
\newcolumntype{L}{>{$}l<{$}}
\newcolumntype{C}{>{$}c<{$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{\textwidth}

\begin{tabular*}{\linewidth}{R C L @{\extracolsep{\fill}} R @{\extracolsep{0.2em}} L}
\multicolumn{5}{c}{(a) Propagation Rules} \\[0.5em]
% 
% Lambda
% 
\downa{\Gamma \vdash A \to B}{\lambda x: A.1. t} &
\step &
\lambda x : A.2. \downa{\Gamma, A \vdash B}{t}
& \textrm{\sc{Propagate-Abs}} & \downarrow
\\
\lambda x : A.1 \upa{\Gamma, A \vdash B}{t} 
& \step &
\upa{\Gamma \vdash A \to B}{\lambda x : A.2. t}
& \textrm{\sc{Propagate-Abs}} & \uparrow
\\[0.5em]
% 
% App
% 
\downa{\Gamma \vdash B}{t_1 \; t_2}
& \step &
\downa{\Gamma \vdash id \to B}{t_1} \; \downa{\Gamma \vdash id}{t_2}
& \textrm{\sc{Propagate-App}} & \downarrow
\\
\upa{\Gamma \vdash A \to B}{t_1} \; t_2
& \step &
\upa{\Gamma \vdash B}{t_1 \; \downa{\Gamma \vdash A}{t_2}}
& \textrm{\sc{Propagate-App}} & \uparrow 1
\\
t_1 \; \upa{\Gamma \vdash A}{t_2}
& \step &
\upa{\Gamma \vdash id}{\downa{\Gamma \vdash A \to id}{t_1} \; t_2}
& \textrm{\sc{Propagate-App}} & \uparrow 2
\\[0.5em]
% 
% Var
% 
\downa{... x : T ... \vdash id}{x}
& \step &
\upa{id \vdash T}{x}
& \textrm{\sc{Propagate-Var}} & \downarrow 1
\\
\downa{id \vdash T}{x}
& \step & \upa{... x : T ... \vdash id}{x}
& \textrm{\sc{Propagate-Var}} & \downarrow 2
\end{tabular*}

\caption{Propagation rules}
\label{subfig:rules:propagation}

\end{subfigure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \begin{tabular}{r c l >{\raggedleft\arraybackslash}p{16em}}
% \begin{tabular*}{\linewidth}{R C L @{\extracolsep{\fill}}R}
% % 
% % Lambda propagation rules
% % 
% \downa{\Gamma \vdash A \to B}{\lambda x: A.1. t} &
% \step &
% \lambda x : A.2. \downa{\Gamma, A \vdash B}{t}
% & \textrm{\sc{Propagate-Abs}} \downarrow
% \\
% \lambda x : A.1 \upa{\Gamma, A \vdash B}{t} 
% & \step &
% \upa{\Gamma \vdash A \to B}{\lambda x : A.2. t}
% & \textrm{\sc{Propagate-Abs}} \uparrow
% \\[1em]
% % 
% % App propagation rules
% % 
% \downa{\Gamma \vdash B}{t_1 \; t_2}
% & \step &
% \downa{\Gamma \vdash id \to B}{t_1} \; \downa{\Gamma \vdash id}{t_2}
% & \textrm{\sc{Propagate-App}} \downarrow
% \\
% \upa{\Gamma \vdash A \to B}{t_1} \; t_2
% & \step &
% \upa{\Gamma \vdash B}{t_1 \; \downa{\Gamma \vdash A}{t_2}}
% & \textrm{\sc{Propagate-App}} \uparrow 1
% \\
% t_1 \; \upa{\Gamma \vdash A}{t_2}
% & \step &
% \upa{\Gamma \vdash id}{\downa{\Gamma \vdash A \to id}{t_1} \; t_2}
% & \textrm{\sc{Propagate-App}} \uparrow 2
% \\
% \downa{... x : T ... \vdash id}{x}
% & \step &
% \upa{id \vdash T}{x}
% & \textrm{\sc{Propagate-Var}} \downarrow 1
% \\
% \downa{id \vdash T}{x}
% & \step & \upa{... x : T ... \vdash id}{x}
% & \textrm{\sc{Propagate-Var}} \downarrow 2
% \end{tabular*}
% % \vspace{-1em}
% \caption{Propagation rules}
% \label{subfig:rules:propagation}
% % \vspace{1em}
% \end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{\textwidth}
\vspace{-1em}
\begin{center}
\begin{align*}
\\ &
\downa{\Delta \vdash \plusdiffs{A \to}{B}{}}{t}
\step
\lambda x : A . \downa{\plusdiffs{}{\Delta}{, x : A} \vdash B}{t}
& \textrm{\sc{Insert-Abs}} \downarrow
\\ &
\downa{\Delta \vdash \minusdiffs{A \to}{B}{}}{\lambda x : A. t}
\step
\downa{\minusdiffs{}{\Delta}{, x : A} \vdash B}{t}
& \textrm{\sc{Delete-Abs}} \downarrow
\\ &
\lambda x : A. \upa{\Gamma, A \vdash \plusdiffs{+ A \to}{B}{}}{t}
\step
\upa{\Gamma \vdash A \to B}{\downa{\minusdiffs{}{\Gamma}{, - A} \vdash id}{t}}
& \textrm{\sc{Delete-Abs}} \uparrow
\\ & &
% App alteration rules
\\ &
\upa{\Delta \vdash \plusdiffs{A \to}{B}{}}{t}
\step
\upa{\Delta \vdash B}{t \; ?}
& \textrm{\sc{Insert-App}} \uparrow
\\ &
\upa{\Gamma \vdash \minusdiffs{A \to}{B}{}}{t_1} \; t_2
\step
\upa{\Gamma \vdash B}{\ghostapp{t_1}{\; \downa{\Gamma \vdash id}{t_2}}}
& \textrm{\sc{Comment-App}} \uparrow
\\ &
\downa{\Gamma \vdash \plusdiffs{A \to}{B}{}}{t_1 \; \s{? : A}}
\step
\downa{\Gamma \vdash id \to B}{t_1}
& \textrm{\sc{Delete-App}} \downarrow
\\ & &
\\ &
% \downa{... - x : T ... \vdash id}{x}
\downa{C \ohchole{\minusdiffs{}{...}{x : T}} \vdash id}{x}
\step
\ghostvar{x}{T}
\jacob{\textrm{TODO: notation here?}}
& \textrm{\sc{Local-To-Free}}
\\ &
\downa{... + x : T ... \vdash id}{\ghostvar{x}{T}}
\step
x
& \textrm{\sc{Free-To-Local}}
\end{align*}
\end{center}
\vspace{-1em}
\caption{Alteration rules}
\label{subfig:rules:alteration}
\vspace{1em}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{\textwidth}
\vspace{-1em}
\begin{center}
\begin{align*}
&
% \downa{id \vdash id}{t}
% \step
% t
% & \textrm{\sc{Identity}} \downarrow
% \\ &
% \upa{id \vdash id}{t}
% \step
% t
% & \textrm{\sc{Identity}} \uparrow
\downa{id \vdash id}{t}
\step
t
\hspace{5em}
\upa{id \vdash id}{t}
\step
t
& \textrm{\sc{Identity}}
%%%%
% \\ &
% \downa{\Gamma \vdash T}{t} \step \errorboundary{A}{B}{\downa{\Gamma \vdash id}{t}} \textrm{ if $T \ne id$, $\diffsto{A}{T}{B}$ and $t$ is a neutral form}
% & \textrm{\sc Neutral} \uparrow
% \\ &
% C[\upa{\Gamma \vdash T}{t}] \step c[\upa{\Gamma \vdash id}{\errorboundary{B}{A}{t}}]
% \textrm{ if $t$ is a neutral form and $C \ne \square \; t_2$}
% & \textrm{\sc Neutral} \downarrow
\\ &
\downa{\Gamma \vdash T}{t} \step \errorboundary{A}{B}{\downa{\Gamma \vdash id}{t}}
\hspace{2em}
C \ohchole{\upa{\Gamma \vdash T}{t}} \step C \ohchole{\upa{\Gamma \vdash id}{\errorboundary{B}{A}{t}}}
& \textrm{\sc Neutral}
\\ &
\hspace{4em} \textrm{ where $\diffsto{A}{T}{B}$, $t$ is a neutral form, and $C \ne \clasp{} \; t_2$}
\\ &
\downa{\Gamma \vdash id}{\upa{id \vdash T}{t}} \step \upa{id \vdash T}{\downa{\Gamma \vdash id}{t}}
\hspace{2em}
\downa{id \vdash T}{\upa{\Gamma \vdash id}{t}} \step \upa{\Gamma \vdash id}{\downa{id \vdash T}{t}}
& \textrm{\sc Interchange}
\\ &
\downa{\Delta \vdash \delta}{t} \step \errorboundary{A}{B}{t}
\hspace{3em}
\upa{\Delta \vdash \delta}{t} \step \errorboundary{B}{A}{t}
& \textrm{\sc Error}
\\ &
\hspace{4em} \textrm{ where $\diffsto{A}{T}{B}$, and no other rules apply}
&
\end{align*}
\end{center}
\caption{Diff boundary rules}
\label{subfig:rules:other}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\caption{The diff propagation rules of Pantograph on $\lambda$ abstractions, applications, and variables.}
\label{fig:rules}
\endgroup
\end{figure}

==> userstudy-v1.tex <==
\subsection{User Study}
\label{sec:userstudy}

(This section is a very rough draft)

We have shown that our zipper editing and typed refactoring systems allow semantically meaningful edits which preserve the grammar and typing of the program. In order to demonstrate that the system is usable and doesn't impede the ability to edit code, we ran a user study in which participants solved simple functional programming problems in both Pantograph and a text editor.
%

We recruited 13 participants (P1-P13) from an advanced undergraduate functional programming course at our institution. The participants were given a 50 minute tutorial session on Pantograph, in which they completed a series of exercises and were given individual help when needed. The participants then completed 12 test problems, half in Pantograph and half in a text editor. The text editor was custom designed for the study to give syntax highlighting and in place type error messages for the same simple functional language used in Pantograph. The participants were evenly divided into Groups A and B, which did the first half the problems in Pantograph and Text respectively, and then switched editors for the second half of the problems (TODO: confirm details).

Six of the twelve problems were taken (with small adjustments to fit our system) from prior works (TODO: Tylr, MPS study). Following these prior works, these problems asked the users to transcribe or edit a program to replicate a given example program. These problems were designed to require nontrivial but realistic edits to an existing program. These problems included for example instructions to move a let binding locally into a definition.

We also investigated the effeciveness of Pantograph on programming problems. We designed the other six problems to test simple functional programming ability. These problems did not give exact solutions to be copied, and therefore required some degree of understanding and thinking about the code. They were designed to test common programming situations.
These problems included for example implementing a function to reverse a list, and generalizing a function to take a new argument.

Overall in our investigation, we were interested in three main questions:

\begin{itemize}
    \item Can we overall teach undergraduates with functional programming experience to use Pantograph effectively?
    \item
    Is Pantograph's rigid focus on semantically structured edits more helpful or harmful depending on a participant's skill at functional programming?
    \item Is Pantograph's style of structure editing more useful for coding problems than for transcription and prescribed edit problems?
\end{itemize}

% Two of the participants (P1 and P6) skipped all of the coding problems in both sections.
% While it is clear to us that these participants were not able to effectively solve problems in Pantograph, is it not clear that they were able to in a text editor either. In addition, in the case of P1, we miscommunicated our instructions about skipping problems. As a result, while we count these two participants among the seven for which Pantograph was much slower, we exclude them from the following analysis.

Participants were told that they could skip a problem if they felt that they had been stuck on it for a long time and wouldn't be able to solve it. For the most part this was rare, except for two participants (P1 and P6) who skipped at least half of the problems on both the text and Pantograph sections, including all of the coding problems. We also neglected to follow our protocol and told P1 to skip a problem that they were stuck on for a long time. We exclude P1 and P6 from the following analysis due to lack of data, but we are confident that they represent examples of participants for which Pantograph did not work well.

Additionally, there were five instances where our test cases passed an incorrect solution - we discarded these data points. This left us with 126 data points, three of which were skipped problems (one in Pantograph and two in the text editor). For these, for the purposes of the following analysis, we assumed that they took the maximum amount of time that any participant took on that problem.

\includegraphics[scale=0.2]{userstudy/boxplots.png}

\includegraphics[scale=0.4]{userstudy/combinedboxes.png}

\paragraph{Relation between user and pantograph}

We investigated the relationship between how fast a user solved problems in Pantograph and in the text editor. We fit a model to the data with one parameter for each problem, and one for each participant-editor pair. Each point on this plot is a participant, and the coordinates show the Pantograph and Text coefficients for that participant.

\includegraphics[scale=0.7]{userstudy/participantplot.png}


There is a clear trend - the participants who were the fastest in text had similar times between text and pantograph. However, the participants who were slower with text were many times slower with Pantograph. There is one outlier - P12, who skipped two of the text problems due to confusion with syntax and type errors.

\jacob{There is a clear trend, but is it interesting? Can we conclude anything from it?}

==> userstudy-v2-prereview.tex <==
\section{User Study}
\label{sec:userstudy}


% % Trying a different way of writing this which gets across that
% % we are testing if people can learn the paradigm, rather than the UI
% The focus of this paper is the diff calculus and the editing paradigm that it enables,
% and we have already shown by example its theoretical value. However, it remains to be shown whether programmers can learn to think in the paradigm required by Pantograph and whether these paradigms lend themselves to an effective user interface.
% % Therefore, we designed a study in which we 
% Therefore we implemented our zipper editing and typed editing paradigms in a structure editor usable in a web app, and in this section we empircally investigate how Pantograph can be taught and used for a collection of basic programming tasks.
% We conducted a user study in which participants were first given an introductory tutorial on using Pantograph, and then timed on a series of programming exercises using either Pantograph or a text editor.

% [OLD] While the focus of this paper is the diff calculus which powers the abstractions that Pantograph provides, such abstractions also need to facilitate enhanced user experience. 
While Pantograph's diff calculus is the primary focus of this paper, such abstractions also need to enhance user experience.
%
% [OLD] However, a thorough empirical comparison of the effectiveness of typed editing compared to other structure editors or traditional text editors would be a herculean task---way beyond the scope of this work.
To convincingly establish the effectiveness of a particular editor, one would need to undertake a thorough empirical comparison of its effectiveness compared to other editors, but such a herculean task is way beyond the scope of this work.
%
Instead, in this section we empirically investigate whether programmers can learn to think and program in the paradigm presented in this paper:
we describe a user study in which participants were first given a short introductory tutorial on using Pantograph, before being asked to complete a series of basic programming tasks using either Pantograph or a text editor.

\paragraph{Participants}

% [OLD] We implemented the Pantograph prototype to use an ML-like strongly-typed and functional programming language, so we sought participants with prior experience with such languages.
We sought participants with prior experience with strongly-typed and functional programming languages, so
we recruited 13 students (11 male, 1 female, 1 unstated; ages 19-25) from \emph{an upper level functional programming course} \footnote{Details elided from this version for anonymization purposes.}, and offered participants a \$30 compensation.
Recruitment materials included a link to Pantograph, and one participant used it recreationally before the study.

%\begin{itemize}
%    \item Gender: 1 female and 11 male

%    \item 2 participants used Pantograph previously\footnote{The Pantograph tutorial was available online publicly before the user study, and the link to it was shared in the invitation email.}
%    \item Age: average 20 years, median 20.66 years
%    \item Year in university: median 3 years, average 2.92 years
%    \item Subjective experience with functional programming (on a scale from 1-5): median 3, average 3.13
%\end{itemize}

% , and conducted the user study at the end of the semester when all students in the class should have had ample opportunity to become familiar with strongly-typed functional programming.
%
% \leo{Not sure all of these are needed or that we have space for them}
%We recruited by making an announcement at the end of a class session and by sending an invitation email to the class's email list.
%As incentive, we mentioned in the invitation that each person would be rewarded \$\todoInline{payout amount} for participation.
% We conducted the user study in two independent sessions on two different days in order to provide more opportunity for those interested to join,
% and ended up recruiting 13 participants in total with a \leo{is there any of these that are actually relevant?}.
% 
%the following demographics (one participant did not fill out the demographics survey): 
%\begin{itemize}
%    \item Gender: 1 female and 11 male

%    \item 2 participants used Pantograph previously\footnote{The Pantograph tutorial was available online publicly before the user study, and the link to it was shared in the invitation email.}
%    \item Age: average 20 years, median 20.66 years
%    \item Year in university: median 3 years, average 2.92 years
%    \item Subjective experience with functional programming (on a scale from 1-5): median 3, average 3.13
%\end{itemize}
% TODO: interesting notes about demographics

% \begin{center}
%     \begin{tabular}{|r||c|c|}
%         \hline
%         Gender & Female & Male \\\hline
%         No. of Participants & 1 & 11
%         \\\hline
%     \end{tabular}
%     \hspace{1em}
%     \begin{tabular}{|r||c|c|c|}
%         \hline
%         Year in School      & 2 & 3 & 4 \\\hline
%         No. of Participants & 4 & 5 & 3
%         \\\hline
%     \end{tabular}
%     \\
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
% \end{center}

\paragraph{Editors and Tasks}

We designed a version of Pantograph \footnote{Available \href{https://pantographeditor.github.io/pantograph-2024-user-study-tutorial/}{here} (anonymized link)} and a text editing environment, both using a simple ML-style programming language, for the study.
The text editor was based on Monaco~\cite{monaco}, the library behind the popular editor Visual Studio Code~\cite{vscode}. We augmented Monaco with syntax highlighting, automatic type-checking, and inline typing diagnostics.
Further, we designed software to conduct the study, available
\href{https://pantographeditor.github.io/pantograph-2024-user-study/}{here} (anonymous link).

Each participant solved the same sequence of 12 tasks (T1-T12). The tasks were designed in six pairs and each participant solved one task from each pair in each editor.
Four tasks (T1, T2, T7, T8) were taken from a prior study on Tylr~\cite{tylr}, asking participants to transcribe a given program and then edit it into a second given one. 
Another pair of tasks (T5, T11) was inspired by a prior study of MPS~\cite{mpsstudy}, in which participants were instructed to fix definitions of a common mathematical law given a correct version to copy.
Because we also wanted to test each participant's ability to program using our typed editing paradigm rather than merely copy given code, we designed six programming tasks: two tasks to implement a function using a given fold function (T3, T9), two tasks to generalize a given function implementation in a specified way (T4, T10), and two tasks to implement a simple recursive function over a list (T6, T12).

% In the study, each participant did half the tasks using Pantograph and half the tasks using Monaco rather than a within-subjects method: since many of the tasks required the participants to decide on how to approach the task at a higher level than just transcription,we would expect to see a relatively large learning effect on the second time doing a task even with a different editor. 

\paragraph{Procedure}

% and participants could ask the study organizers any questions.
The participants were given a 1-hour tutorial on Pantograph consisting of interactive examples and exercise which explained typed tree editing, zipper editing and selections, and type boundaries.
During the tutorial, we actively answered questions and assisted participants.
% The major topics covered were: mouse interactivity, typed holes, insertion, deletion, selection, cutting, pasting, and type boundaries.
Additionally, each participant was given 5 minutes to familiarize themselves with the text editor.

After the tutorial, the participants were randomly divided into two groups. 
% The problems were designed to some in similar pairs, where each participant would do one problem from each pair in each editor.
Group A solved the first six tasks in Pantograph and the last six tasks in the text editor, while group B used the editors in the reverse order.
While solving tasks, participants were allowed to ask questions about the language or editor but not about how to solve the task.
When a participant's code passed a task's test suite, the software indicated that they could continue to the next task.
Participants were informed that they should skip any task that they thought they couldn't finish or was taking them too long.


\paragraph{Results}

The user study yielded roughly 10 hours of screen recordings.
In all, 156 tasks were attempted by the participants.
Two participants (one in Group A and one in Group B) skipped at least six tasks, including all of the programming tasks in both editors
---
% in any case it is clear that Pantograph did not work well for these participants, and
we chose to omit their data from the following analysis, although we discuss this issue further in the limitations section.
Further, we discarded the data points (4 in Pantograph and 2 in text) where our test suite passed an incorrect solution.
This left us with 124 data points on tasks, 121 of which were solved and 3 of which were skipped.
%

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{userstudy/alldata_v11.png}
    % \includegraphics[width=\textwidth]{userstudy/measurements-final-box-scatter-v2.png}
    \caption{Task durations (in seconds) split by editor. For each task, Pantograph times are on the top in orange, and text times are on the bottom in blue. Tasks that participants chose to skip are marked as a red `X'. }
    %\jacob{There is still something wrong with the data. The Xs shouldn't be overlapping any other points if it was done correctly.}}
    \label{fig:alldata}
    % \jacob{TODO: key?} \jacob{TODO: I am suspicious of how two of the Xs overlap other points. Something is wrong with the data there.}}
\end{figure}

\begin{figure}
    \centering
    % \includegraphics[width=0.5\linewidth]{userstudy/perparticipantplot.png}
    \includegraphics[width=0.5\linewidth]{userstudy/duration_ratios_v2.png}
    % \caption{\jacob{This is a temporary picture, we will make a nicer looking one.}}
    \caption{
    % Task duration ratios for each participant. The horizontal coordinate is the geometric mean, over each task the participant used Pantograph, of the ratios of their duration vs the average duration among all participants on that task. The vertical coordinate is the geometric mean, over each task the participant used Monaco, of the ratio of their duration vs the average duration among all participants on that task.
    % Error bars along both dimensions span the geometric mean divided by 1 geometric standard deviation to the geometric mean multiplied by 1 geometric standard deviation.
    % The dotted line marks the line $y = x$; the closer a participant's point is to $y = x$, the more similar their performance in Pantograph and Monaco.
    % 
    % 
    % 
    % 
    % Average pantograph and text task times and variance for each participant.
    % Task times are given as a ratio to average time taken, as a geometric mean over all tasks.
    % Horizontal and vertical lines indicate 1 standard deviation.
    % 
    % 
    % 
    Geometric mean and variance of relative task times for each participant (denoted as a dot), and for each editor. The dashed line shows parity between the editors --- participants below the line solved tasks slower in Pantograph then the text editor. One standard deviation is shown as horizontal and vertical lines.
    }
    \label{fig:duration-ratios}
\end{figure}

% \subsection{Summary of data}
%\paragraph{Findings}

% All of this data is presented in Figure~\ref{fig:alldata}.
Figure~\ref{fig:alldata} shows the duration of each task for each editor.
Overall, Pantograph was slower than the text editor for most tasks.
% [OLD] measured by taking the ratio of the average durations of each editor for a task, and then the geometric mean of these ratios across tasks.
It was $1.4\times$ slower on average overall, measured as the geometric mean of the ratio between the average duration of each editor on each task.
% Figure ~\ref{fig:duration-ratios} shows for each participant the geometric means of the ratio between their duration for each editor on each task to the average duration on that task.

% % 
In order to view these task durations by participant, we need a way to compare times across different tasks. We define a participant's \emph{relative task time} as the ratio of their time to the average time taken on that task.
% In order to also compare task times by participant across multiple tasks, we first define a relative task time as the ratio of the task time to the average time taken to complete that task by all participants.
We plotted the average relative task time in each editor for each participant in Figure~\ref{fig:duration-ratios}.
To account for skipped tasks in this calculation, we used the maximum time taken for that task by any participant.
% Most (8) of the participants performed similarly in both editors, while a few (3) clustered around significant slower performance in Pantograph.
% HENRY: this might be too strong a claim? can't really quantify it, its just a sparse clustering
% Jacob:  Yes it is way too strong, we absolutely can't claim that.
Some of the participants performed similarly in both editors, while some performed significantly more slowly in Pantograph than the text editor.
% Participants that performed faster in Pantograph tended to perform more similarly on both editors,
% and participants that performed slower in Pantograph tended to perform slower in the text editor as well.
Overall, most of the participants in the study were able to effectively solve the tasks using Pantograph.

% In particular, participants who were much faster than average at solving problems in the text editor tended to be 

% \paragraph{Main Observations.}
% From the data presented in figure \ref{fig:alldata}, we make the following observations:
% \begin{enumerate}
% \item
% In 6 out of 12 tasks, the average task duration using Pantograph was at most 1 standard deviation higher than the average task duration using Monaco.

% \item
% In 10 out of the 12 tasks, the average task duration using Pantograph was longer than the average task duration using Monaco.
% In 6 out of those 10 tasks, the mean Pantograph duration was more than 1 standard deviation higher than the mean Monaco duration.
% In 4 out of those 6 tasks, the mean Pantograph duration was more than 2 standard deviations higher than the mean Monaco duration.

% \item
% In 2 out of the 12 tasks, the average task duration using Pantograph was shorter than the average task duration using Monaco. 
% Both of these tasks were centered around using the \code{fold} function to fold-left over a list.

% \item 
% The significant right-tail outlier for using EDITOR on the TASK task was influenced by a confusion about shadowing built-in names.\footnote{the implementation of EDITOR did not allow shadowing of built-in names, but in retrospect this is a bug.}
% \todo{TODO: double-check this -- was this in Pantograph or Monaco, and which task was it again????}

% \item
% The task duration variance was on average much higher among Pantograph uses than among Monaco uses.
% \todo{specific average variance for Pantograph vs Monaco}
% \end{enumerate}

% Overall, this study demonstrates that several of the recruited students were able to learn via a roughly 1-hour tutorial how to use Pantograph to complete the collection of editing tasks within a reasonable\todoInline{how to professionally qualify this?} amount of time. 
% However, they rarely demonstrated more efficient use of Pantograph than Monaco, in terms of task duration.
% Additionally, many of the recruited students had significant issues using Pantograph.

% % TODO: finalize wording and perhaps include specific examples if we have space
% % TODO: include references to specific instances of each issue (participant-task pairs)
% \paragraph{Issues in Pantograph.}
% \begin{itemize}
% % \item Didn't realize how to or the need to dig the top-level type hole if it became unified with an unwanted type
% \item Editing a function definition in a way that would not ultimately be helpful for completing the task could modify how the function is used at the call cites in tests, which created more issues for the user to resolve later than they would have to resolve in Monaco
% \item Dug and rewrote expression rather than cut+paste
% % \item Confusion about where to click to place the cursor at an expression or click+drag to select a one-hole context
% \item After accidentally or mistakenly modifying the type of a function, confusion about how to revert that change or handle its consequences
% \item Seemed to get confused when a hole was a different type from what they expected, and what they indented to put there didn't fit (but this could be due to confusion about how the program is working rather than how Pantograph is forcing them to interact with it)
% % \item Confusion about where to click and what query to make in order to insert a new function argument.
% \todo{more issues}
% \end{itemize}

% % \paragraph{Issues in Monaco.}
% % \begin{itemize}
% % \item Sometimes assumed the availability of language features that were not implemented, and since Monaco only gives them general parsing feedback, it could be hard to infer what syntax was available
% % \item Sometimes forgot minor syntax features, such as the ``\code{|}'' between the branches of a \code{match} expression or the ``\code{in}'' in a \code{let} expression.
% % \todo{more issues}
% % \end{itemize}

% \paragraph{Usage Examples of Pantograph.}
% Although there were many issues, there were also many instances of participants using Pantograph to edit effectively.
% \todo{some examples of how Pantograph was used well}

\paragraph{Limitations}
% % BEGIN JACOB
% Our study has several limitations.
While the tasks in our study were intended to represent realistic programming scenarios, the results may not generalize to real world programming in a fully developed system that the participants were familiar with.
Further, the participants were aware that we made Pantograph, which has been shown to cause bias \cite{biasstudy}.
Unlike prior studies on structure editors such as~\citet{tylr, teentylr, mpsstudy} which focus on transcription tasks, we included programming tasks.
Although we intended the tasks to be easy enough to complete in the time allotted for the study, two participants were still not able to complete any of these coding tasks in either editor, getting stuck on an early problem and then quickly skipping later problems.
As we had not planned task time limits beforehand we decided on our problem skipping protocol during the study, and it is possible that this design flaw influenced the participant's decisions to skip problems.
Regardless of this flaw, it is difficult to design realistic software development tasks which are attainable in the span of a controlled user study.
We leave the development of techniques capable of evaluating structure editing paradigms on real software development for future work.
% % END JACOB
%
%
% Henry's version
% 
% Our study design has several limitations.
% The participants were aware that we made Pantograph, which has been shown to cause bias \cite{biasstudy}.
% Additionally, we decided on our task-skipping protocol during the study, and it is possible that this design flaw influenced the participant's decisions to skip problems.
% We intended the tasks to resemble realistic programming scenarios, in contrast to prior studies such as ~\citet{tylr, teentylr, mpsstudy} which focus on transcription tasks, but also to be easily completable in the time allotted for the study after only one hour of tutorial.
% Even so, two participants did not complete any of the coding tasks in either editor.
% This suggests that it is difficult to design a study that generalizes to real-world programming while still being feasible  for recruits to complete.
% We leave the development of techniques capable of evaluating structure editing paradigms on real software development to future work.
% END henry's version

==> well-typed-edits-first-example.tex <==
\section*{Well typed editing - a first example}
\label{sec:welltyped}

\henry{This is old, was converted into simple first explanation in section \ref{sec:typed-editing}}.

To begin, lets look at how our typed editing system works on a standard simple lambda calculus, with typed holes

\begin{align*}
t ::= \lambda x . t \pipe t \; t \pipe x \; \pipe ?
\hspace{3em}
T ::= T \to T \pipe Int
\hspace{3em}
\Gamma ::= \emptyset \pipe \Gamma, x : T
\end{align*}

\begin{align*}
\inferrule{
    \Gamma, x : T_1 \vdash t : T_2
}{
    \Gamma \vdash \lambda x . t : T_1 \to T_2
}
\hspace{3em}
\inferrule{
    \Gamma \vdash t_1 : T_1 \to T_2
    \\
    \Gamma \vdash t_2 : T_1
}{
    \Gamma \vdash t_1 \; t_2 : T_2
}
\hspace{3em}
\inferrule{
    x : T \in \Gamma
}{
    \Gamma \vdash x : T
}
\hspace{3em}
\inferrule{
}{
    \Gamma \vdash ? : T
}
\end{align*}

From our grammars of types and contexts, we may construct grammars of type diffs $C$ and contexts diffs $\Delta$

$$
d ::= d \to d \pipe + T \to [d] \pipe - T \to [d]
$$

$$
\Delta ::= \emptyset \pipe \Delta, x:d \pipe + [\Delta], x : t \pipe - [\Delta], x : t 
$$


The judgement $t_1 \xrightarrow{d} t_2$ means that $d$ is a diff between $t_1$ and $t_2$. For example, we can construct a diff which adds two arguments into a function type:

$$
T_1 \to T_4 \xrightarrow{T_1 \to + T_2 \to [+ T_3 \to [T_4]]} T_1 \to T_2 \to T_3 \to T_4
$$


\subsection{Typed program edits}

Using these type and context diffs, we may now form the judgement $\Delta \vdash C$, which describes how the type and context of a term has been edited.
We extend our grammar of terms to include \emph{diff boundaries}, which propagate diffs up and down:

$$
t ::= \textcolor{gray}{\lambda x . t \pipe t \; t \pipe x \; \pipe ?} \pipe \downarrow \s {t}_{\Delta \vdash C} \pipe \uparrow \s{t}_{\Delta \vdash C}
$$

The two new forms can be given typing rules

\begin{align*}
\inferrule{
    \Gamma_1 \xrightarrow{\Delta} \Gamma_2
    \\
    T_1 \xrightarrow{C} T_2
    \\
    \Gamma_1 \vdash t : T_1
}{
    \Gamma_2 \vdash \downarrow \s{t}_{\Delta \vdash C} : T_2
}
\hspace{3em}
\inferrule{
    \Gamma_1 \xrightarrow{\Delta} \Gamma_2
    \\
    T_1 \xrightarrow{C} T_2
    \\
    \Gamma_1 \vdash t : T_2
}{
    \Gamma_2 \vdash \uparrow \s{t}_{\Delta \vdash C} : T_1
}
\end{align*}

This can be propagated with smallstep rules

% \jacob{maybe at this point only show the down rules,
% and leave the up rules to the full generalization?}

$$
    \downarrow\s{\lambda x . t}_{\Delta \vdash C_1 \to C_2}
        \; \leadsto \;
    \lambda x . \downarrow \s{t}_{\Delta, x : C_1 \vdash C_2}
$$
% $$
%     \lambda x . \uparrow \s{t}_{\Delta, x : C_1 \vdash C_2}
%         \; \leadsto \;
%     \uparrow \s{\lambda x . t}_{\Delta \vdash C_1 \to C_2}
% $$
$$
    \downarrow \s{t_1 \; t_2}_{\Delta \vdash C_2}
        \; \leadsto \;
    \downarrow \s{t_1}_{id \to C_2} \; \downarrow \s{t_2}_{\Delta \vdash id}
$$
% $$
%     \uparrow \s{t_1}_{\Delta \vdash C_1 \to C_2} \; t_2
%         \; \leadsto \;
%     \uparrow \s{t_1 \; \downarrow \s{t_2}_{\Delta \vdash C_1}}_{\Delta \vdash C_2}
% $$
% $$
%     t_1 \; \uparrow \s{t_2}_{\Delta \vdash C_1}
%         \; \leadsto \;
%     \uparrow \s{\downarrow \s{t_1}_{\Delta \vdash C_1 \to id} \; t_2}_{\Delta \vdash id}
% $$
$$
    \downarrow \s{x}_{\Delta \vdash id}
        \; \leadsto \;
    \uparrow \s{x}_{id \vdash \Delta(x) }
$$

Each of the smallstep rules preserves well-typedness.

Now, lets look at an example of using typechanges in practice. (This is maybe a bad example, because our editor won't propagate it back up like this. But I liked it because it works with only propagation rules, which is what we have at this point)

\begin{center}
\begin{tabular}{ c c c }
 & $\downarrow \s{\lambda x . x}_{\emptyset \;\; \vdash \;\; (+ Int \to [Int]) \to Int}$ \\ 
 $\leadsto$ & $\lambda x . \downarrow \s{x}_{\emptyset, \; x : (+ Int \to [Int]) \;\; \vdash \;\; Int}$ \\
 $\leadsto$ & $\lambda x . \uparrow \s{x}_{\emptyset, \; x : Int \to Int \;\; \vdash \;\; + Int \to [Int]}$ \\
 % $\leadsto$ & $\uparrow \s{\lambda x . x}_{\emptyset \;\; \vdash \;\; (Int \to Int) \to (+ Int \to [Int])}$ \\ 
\end{tabular}
\end{center}

We begin with an identity function of type $Int \to Int$. We have a change applied to this term, which adds a higher-order argument to the input type. The diff boundary steps into the lambda, and the insertion is not in the context diff. The rule then flips direction at the variable; now the insertion is back in the type position. Finally, the boundary steps up through the lambda again. In the end, the system has discovered that to change the input type of the lambda, the output type must also change.

In reality, one may not want this behaviour. For example, in Pantograph we added the following rule:


